Explaining Black-Box Algorithms Using Probabilistic Contrastive Counterfactuals

There has been a recent resurgence of interest in explainable artificial intelligence (XAI) that aims to reduce the opaqueness of AI-based decision-making systems, allowing humans to scrutinize and trust them. Prior work in this context has focused on the attribution of responsibility for an algorithm's decisions to its inputs wherein responsibility is typically approached as a purely associational concept. In this paper, we propose a principled causality-based approach for explaining black-box decision-making systems that addresses limitations of existing methods in XAI. At the core of our framework lies probabilistic contrastive counterfactuals, a concept that can be traced back to philosophical, cognitive, and social foundations of theories on how humans generate and select explanations. We show how such counterfactuals can quantify the direct and indirect influences of a variable on decisions made by an algorithm, and provide actionable recourse for individuals negatively affected by the algorithm's decision. Unlike prior work, our system, LEWIS: (1)can compute provably effective explanations and recourse at local, global and contextual levels (2)is designed to work with users with varying levels of background knowledge of the underlying causal model and (3)makes no assumptions about the internals of an algorithmic system except for the availability of its input-output data. We empirically evaluate LEWIS on three real-world datasets and show that it generates human-understandable explanations that improve upon state-of-the-art approaches in XAI, including the popular LIME and SHAP. Experiments on synthetic data further demonstrate the correctness of LEWIS's explanations and the scalability of its recourse algorithm.

==> app.tex <==
\section{Appendix}
\label{sec:apx}

First, we
prove the following lemma:

\begin{lemma}\label{lemma:ns} The following statement holds:
  \begin{align}
    NS(V \mid \mb k)
    &= \pr(O_{V\leftarrow v}=1 \mid  \mb k)-\pr(O_{V\leftarrow v'}=1 \mid \mb k)+
      \pr(O_{V\leftarrow v}=0,O_{V\leftarrow v'}=1 \mid  \mb k) \label{eq:lemma:ns}
  \end{align}
\end{lemma}

\begin{proof} The following two equations follow from the law of total probability. 
  \begin{align}
    &  \ \pr(O_{V\leftarrow v}=1,\mb k)= \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=1,\mb k) +\pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k) \label{eq:lemma:proof:first}\\
    &\pr(O_{V\leftarrow v'}=1,\mb k)= \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=1, \mb k) +\pr(O_{V\leftarrow v}=0,O_{V\leftarrow v'}=1, \mb k) \label{eq:lemma:proof:second}
  \end{align}

  We rearrange Equations~\eqref{eq:lemma:proof:first} and
  \eqref{eq:lemma:proof:second} as follows:
    \begin{align}
      \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k)
      &=  \pr(O_{V\leftarrow v}=1,\mb k) -  \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=1,\mb k) \label{eq:lemma:proof:third}\\
      \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=1, \mb k)
      &= \pr(O_{V\leftarrow v'}=1,\mb k) - \pr(O_{V\leftarrow v}=0,O_{V\leftarrow v'}=1, \mb k)  \label{eq:lemma:proof:fourth}
  \end{align}

  By substituting \eqref{eq:lemma:proof:fourth} into
  \eqref{eq:lemma:proof:third}, we get:
  \begin{align}
    \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k)
    &=  \pr(O_{V\leftarrow v}=1,\mb k) -  \pr(O_{V\leftarrow v'}=1,\mb k) +
      \pr(O_{V\leftarrow v}=0,O_{V\leftarrow v'}=1, \mb k)\label{eq:lemma:proof:fifth}
  \end{align}

  We attain equation~\ref{eq:lemma:ns} after dividing
  \eqref{eq:lemma:proof:fifth} by $\frac{1}{\pr(\mb k)}$.
\end{proof}


{\bf Proof of Proposition~\ref{eq:iden:mon:ci}:}{ 


  \begin{align}
    NS(V \mid \mb k)
    &= \pr(O_{V\leftarrow v}=1 \mid  \mb k)-\pr(O_{V\leftarrow v'}=1 \mid \mb k)+
      \pr(O_{V\leftarrow v}=0,O_{V\leftarrow v'}=1 \mid  \mb k) \label{eq:lemma:ns}
  \end{align}
  
  
    \begin{align}
    NS(V \mid \mb k)
    & \leq \pr(O_{V\leftarrow v}=1 \mid  \mb k)-\pr(O_{V\leftarrow v'}=1 \mid \mb k)+
      \pr(O_{V\leftarrow v}=0 \mid  \mb k) \nonumber \\
         &  =  1- \pr(O_{V\leftarrow v'}=1 \mid  \mb k)  \nonumber \\
          &  =  \pr(O_{V\leftarrow v'}=0 \mid  \mb k)
  \end{align}

    \begin{align}
    NS(V \mid \mb k)
    & \leq \pr(O_{V\leftarrow v}=1 \mid  \mb k)-\pr(O_{V\leftarrow v'}=1 \mid \mb k)+
      \pr(O_{V\leftarrow v'}=1 \mid  \mb k)  \nonumber \\
    &  =   \pr(O_{V\leftarrow v}=1 \mid  \mb k)  \
      \label{eq:lemma:ns}
  \end{align}
  
  \begin{align}
    NS(V \mid \mb k)
    &\geq \pr(O_{V\leftarrow v}=1 \mid  \mb k)-\pr(O_{V\leftarrow v'}=1 \mid \mb k) \label{eq:lemma:ns}
  \end{align}

  {\scriptsize   
\begin{align}
\max\Bigg\{0, \pr(O=1 \mid \Do(V=v),  \mb k)-\pr(O=1 \mid \Do(V=v'), \mb k)   \Bigg\}  \leq      NS(V \mid \mb k) \leq  \min
\Bigg\{  \pr(O=1 \mid \Do(V=v), \mb k) , \pr(o' \mid \Do(V=v'), \mb k)\Bigg\}  \nonumber \\
  \end{align}
  }


  \begin{align}
    \pr(O_{V\leftarrow v}=0, v,\mb k)
    &=  \pr(O_{V\leftarrow v}=0, O_{V\leftarrow v'}=0, v,\mb k)
      + \pr(O_{V\leftarrow v}=0, O_{V\leftarrow v'}=1, v,\mb k) \label{eq:prop:first}\\
  \pr(O_{V\leftarrow v'}=0, v,\mb k)
    &=  \pr(O_{V\leftarrow v'}=0, O_{V\leftarrow v}=0, v,\mb k)
      + \pr(O_{V\leftarrow v'}=0, O_{V\leftarrow v}=1, v,\mb k) \nonumber\\
      \label{eq:prop:second2}
  \end{align}

  \begin{align}
\pr(O_{V\leftarrow v'}=0, O_{V\leftarrow v}=1, v,\mb k) &=
     \pr(O_{V\leftarrow v'}=0, v,\mb k) - 
       \pr(O_{V\leftarrow v}=0, v,\mb k)+     \pr(O_{V\leftarrow v}=0, O_{V\leftarrow v'}=1, v,\mb k)  \nonumber \\
     &=    \pr(O_{V\leftarrow v'}=0, \mb k)- \pr(o', v', \mb k) +        \pr(O_{V\leftarrow v}=0, v,\mb k)+  \nonumber \\  & \pr(O_{V\leftarrow v}=0, O_{V\leftarrow v'}=1, v,\mb k) \\
  \end{align}
  
  
  
  
      \begin{align}
\pr(O_{V\leftarrow v'}=0, O_{V\leftarrow v}=1, v,\mb k) & \geq
     \pr(O_{V\leftarrow v'}=0, v,\mb k) - 
       \pr(O_{V\leftarrow v}=0, v,\mb k) \nonumber \\ 
      &= \pr(O_{V\leftarrow v'}=0, \mb k)- \pr(o', v', \mb k) -        \pr(O_{V\leftarrow v}=0, v,\mb k) \nonumber \\ 
      &= \pr(O_{V\leftarrow v'}=0, \mb k)- \pr(o', \mb k)
  \end{align}
  
 
 \begin{align}
\pr(O_{V\leftarrow v'}=0, O_{V\leftarrow v}=1, v,\mb k) & =
     \pr(O_{V\leftarrow v'}=0, v,\mb k) - 
       \pr(O_{V\leftarrow v}=0, v,\mb k)+     \pr(O_{V\leftarrow v}=0, O_{V\leftarrow v'}=1, v,\mb k)  \nonumber \\
     &  \leq   \pr(O_{V\leftarrow v'}=0, v,\mb k) - 
       \pr(O_{V\leftarrow v}=0, v,\mb k)+     \pr(O_{V\leftarrow v'}=1, v,\mb k)  \nonumber \\
     &=  \pr(v,\mb k) - 
       \pr(o', v,\mb k)= \pr(o, v,\mb k)  \nonumber \\
  \end{align}
    
    
      \begin{align}
\pr(O_{V\leftarrow v'}=0, O_{V\leftarrow v}=1, v,\mb k) & =
     \pr(O_{V\leftarrow v'}=0, v,\mb k) - 
       \pr(O_{V\leftarrow v}=0, v,\mb k)+     \pr(O_{V\leftarrow v}=0, O_{V\leftarrow v'}=1, v,\mb k)  \nonumber \\
     &\leq    \pr(O_{V\leftarrow v'}=0, \mb k)- \pr(o', v', \mb k) -        \pr(O_{V\leftarrow v}=0, v,\mb k)+  \pr( O_{V\leftarrow v}=0, v,\mb k) \nonumber \\
     &= \pr(O_{V\leftarrow v'}=0, \mb k)- \pr(o', v', \mb k)
  \end{align}
  
  {\small 
        \begin{align}
\max\Bigg\{0, \frac{\pr(O_{V\leftarrow v'}=0, \mb k)- \pr(o', v', \mb k)}{\pr(O=1, v,\mb k)}  \Bigg\}  \leq  N(V \mid \mb k)\leq  \min
\Bigg\{ \frac{\pr(v,\mb k) - 
       \pr(o', v,\mb k)}{\pr(O=1, v,\mb k)}, \frac{\pr(O_{V\leftarrow v'}=0, \mb k)- \pr(o', v', \mb k)}{\pr(O=1, v,\mb k)}  \Bigg\}  \nonumber \\
  \end{align}
  }
  
$\pr(O_{V\leftarrow v'}=1, \mb k)=\pr(O=1 \mid \Do(V=v'), \mb k)$
  
  {\scriptsize   
\begin{align}
\max\Bigg\{0, \frac{\pr(O=1 \mid \mb k)- \pr(O=1, \mid \Do(V=v'),  \mb k)}{\pr(O=1, v \mid \mb k)}   \Bigg\}  \leq  N(V \mid \mb k) \leq  \min
\Bigg\{ 1, \frac{\pr(O=0, \mid \Do(V=v'), \mb k)- \pr(O=0, v' \mid \mb k)}{\pr(O=1, v \mid \mb k)}  \Bigg\}  \nonumber \\
  \end{align}
  }
  
   %    \begin{align}
   %N(V\mid \mb k) &= \frac{{}\pr(O_{V \leftarrow v'}=0 \mid V=v,  O=1, \mb K=\mb k)
   % \end{align}
  

  \begin{align}
     \pr(O_{V\leftarrow v'}=0, \mb k) =      \pr(O_{V\leftarrow v'}=0, v, \mb k) +      \pr(O_{V\leftarrow v'}=0, v', \mb k) \\
     = \pr(O_{V\leftarrow v'}=0, v, \mb k) +      \pr(O=0, v', \mb k)
  \end{align}

  Equation~\eqref{eq:prop:ns} follows from Lemma~\ref{lemma:ns}, and the fact
  that under the assumption of monotonicity
  $\pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k) = 0$ and under the
  assumption that variables $K$ are non-descendents of $V$
  $\pr(O_{V\leftarrow v}=1,\mb k) = \pr(O=1 \mid \Do(V=v), \mb k)$.


  Equation~\eqref{eq:prop:s} follows from the following derivations. First, we
  use the law of total probability to rewrite
  $\pr(O_{V\leftarrow v}=1, v',\mb k)$ and $\pr(O_{V\leftarrow v'}=1,v',\mb k)$:
  \begin{align}
    \pr(O_{V\leftarrow v}=1, v',\mb k)
    &= \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=1,\mb k, v')
      + \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k, v') \label{eq:prop:first}\\
    \pr(O_{V\leftarrow v'}=1,v',\mb k)
    &= \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=1, \mb k, v')
      + \pr(O_{V\leftarrow v}=0,O_{V\leftarrow v'}=1, \mb k,v') \nonumber\\
  \end{align}

  By substituting \eqref{eq:prop:second2} into \eqref{eq:prop:first}, we get:
  
  
    \begin{align}
  \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k, v')   &=       \pr(O_{V\leftarrow v}=1, v',\mb k)   - \pr(O_{V\leftarrow v'}=1,v',\mb k)+ \pr(O_{V\leftarrow v}=0,O_{V\leftarrow v'}=1, \mb k,v') 
    \label{eq:prop:third}
   \end{align}
   
   
       \begin{align}
  \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k, v')   &\geq      \pr(O_{V\leftarrow v}=1, v',\mb k)   - \pr(O_{V\leftarrow v'}=1,v',\mb k)
\nonumber \\
 & \geq   \pr(O_{V\leftarrow v}=1,\mb k) - \pr(O=1,v,\mb k)  - \pr(O_{V\leftarrow v'}=1,v',\mb k)\nonumber \\
 & =\pr(O_{V\leftarrow v}=1,\mb k) - \pr(O=1,\mb k) 
   \end{align}
   
   
       \begin{align}
  \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k, v')   &\leq       \pr(O_{V\leftarrow v}=1, v',\mb k)   - \pr(O_{V\leftarrow v'}=1,v',\mb k)+ \pr(O_{V\leftarrow v}=0, \mb k,v') \nonumber\\
 &= P(v', \mb k)- \pr(O=1,v',\mb k)= \pr(O=0,v',\mb k)
    \label{eq:prop:third}
   \end{align}
   
   
       \begin{align}
  \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k, v')   &\leq       \pr(O_{V\leftarrow v}=1, v',\mb k)   - \pr(O_{V\leftarrow v'}=1,v',\mb k)+ \pr(O_{V\leftarrow v'}=1, \mb k,v') \nonumber\\
  & = \pr(O_{V\leftarrow v}=1,\mb k) - \pr(O=1,v,\mb k)  - \pr(O=1,v',\mb k)+ \pr(O=1, \mb k,v') \nonumber\\
  & = \pr(O_{V\leftarrow v}=1,\mb k)  - \pr(O=1,\mb k)+ \pr(O=1, \mb k,v') \nonumber\\
  & = \pr(O_{V\leftarrow v}=1,\mb k)  -  \pr(O=1, \mb k,v) 
    \label{eq:prop:third}
   \end{align}
   
     {\scriptsize   
\begin{align}
\max\Bigg\{0, \frac{\pr(O=1\mid \Do(V=v) ,\mb k) - \pr(O=1,\mb k) }{\pr(O=0, v' \mid \mb k)}   \Bigg\}  \leq  S(V \mid \mb k) \leq  \min
\Bigg\{ 1, \frac{\pr(O=1\mid \Do(V=v), \mb k)  -  \pr(O=1,v \mid \mb k)}{\pr(O=0, v' \mid \mb k)}  \Bigg\}  \nonumber \\
  \end{align}
  }
  
  \begin{align}
    \pr(O_{V\leftarrow v}\leq 1,O_{V\leftarrow v'}=0,\mb k, v') &= 
    \pr(O_{V\leftarrow v}=1, v',\mb k) - \pr(O_{V\leftarrow v'}=1,v',\mb k)
    \label{eq:prop:third}
   \end{align}
  
  
  Similarly, we can rewrite:
  \begin{align}
    \pr(O_{V\leftarrow v}=1,\mb k)
    &=\pr(O_{V\leftarrow v}=1,v',\mb k)+\pr(O_{V\leftarrow v}=1,v,\mb k) \\
    &=\pr(O_{V\leftarrow v}=1,v',\mb k)+\pr(O=1,v,\mb k) \label{eq:prop:fourth}
  \end{align}
  which shows that
  \begin{align}
    \pr(O_{V\leftarrow v}=1,v',\mb k) = \pr(O_{V\leftarrow v}=1,\mb k) - \pr(O=1,v,\mb k)
    \label{eq:prop:fifth}
  \end{align}

  We next combine \eqref{eq:prop:third} and \eqref{eq:prop:fifth}:
  \begin{align}
    \pr(O_{V\leftarrow v}=1,O_{V\leftarrow v'}=0,\mb k, v')
    & = \pr(O_{V\leftarrow v}=1, v',\mb k)-\pr(O_{V\leftarrow v'}=1, v', \mb k) \\
    &=\pr(O_{V\leftarrow v}=1,\mid \mb k)-\pr(O=1,v, \mb k)-
      \pr(O_{V\leftarrow v'}=1, v', \mb k) \\
    &=\pr(O_{V\leftarrow v}=1,\mid \mb k)-\pr(O=1,v, \mb k)-
      \pr(O=1, v', \mb k) \\
    & = \pr(O_{V\leftarrow v}=1, \mb k)-\pr(O=1, \mb k) \label{eq:prop:sixth}
  \end{align}

  We can now prove Equation~\eqref{eq:prop:s}: 
  \begin{align}
    S(V\mid \mb k)
    &= \pr(O_{V\leftarrow v}=1 \mid V=v', O=0, \mb K=\mb k) \\
    &= \frac{ \pr(O_{V\leftarrow v}=1, V=v', O=0, \mb K=\mb k) }{\pr(V=v', O=0, \mb K=\mb k)}\ \\
    &= \frac{ \pr(O_{V\leftarrow v}=1, V=v', O_{V\leftarrow v'}=0, \mb K=\mb k)}
      {\pr(V=v', O=0, \mb K=\mb k)}   && \texttt{(consistency)}\\
    &= \frac{ \pr(O_{V\leftarrow v}=1, \mb k)-\pr(O=1, \mb k) }{\pr(V=v', O=0, \mb K=\mb k)}
     && \texttt{(from Eq.\eqref{eq:prop:sixth})}\\
    &= \frac{ \pr(O_{V\leftarrow v}=1, \mb k)-\pr(O=1, \mb k) }
      {\pr(V=v', O=0 \mid K=\mb k) \pr(K=\mb k)} \\
    &= \frac{ \pr(O_{V\leftarrow v}=1 \mid \mb k)-\pr(O=1 \mid  \mb k) }
      {\pr(V=v', O=0 \mid K=\mb k)} \\
    &= \frac{ \pr(O=1 \mid \Do(V\leftarrow v)\mb k)-\pr(O=1 \mid  \mb k) }
      {\pr(V=v', O=0 \mid K=\mb k)} && \texttt{(if K is non-decendent of Y)}
  \end{align}

  Equation~\eqref{eq:prop:n} can be proved similarly.
}

==> conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}
\vspace{-2pt}
The proposed system \sys\ generates post-hoc explanations for black-box decision-making algorithms using probabilistic contrastive counterfactuals. \sys\ explains the output of an algorithm globally, locally and contextually in terms of novel probabilistic measures that quantify the extent to which an attribute is necessary and sufficient for an algorithm's decisions. We established conditions under which \sys's scores can be bounded and estimated using historical data. \sys\ further leverages these scores for the problem of generating actionable recourse for producing the desired algorithm outcome in the future.
Experimental evaluation on real and synthetic datasets show that \sys's explanations are coherent with insights from existing work, and validate the correctness of its estimates and the efficiency of its recourse algorithm.

==> cut.tex <==
\subsection{Multivalued Extension} In this section we discuss the extension of necessity score to multivalued features and the sufficiency score to a set of feature. The motivation is to ... 


Let $Dom(V) = \{v_1, v_2, \ldots, v_n\}$, we say an event $V=v_i$ is a necessary and sufficient cause of a positive outcome of algorithm $O=1$ in a context $\mb K= \mb k$ if respectively the following logical conditions hold:
%
\begin{align}
\forall \mb u,   \mb u(V)=v_i \ \land \ \mb u(O)=1 \land \mb u(\mb K)= \mb k  &\implies 
\bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v}(\mb u) =0\\
\forall \mb u,  \bigvee_{v \not =  v_i}  \mb u(V)=v \ \land \ \mb u(O) =0 \land \mb u(\mb K)= \mb k  &\implies   \ O_{V\leftarrow v_i}(\mb u) =1
\label{eq:mpn}
\end{align}
%
These logical implications have the following probabilistic interpretation:
%
\begin{align}
\pr(\bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0 \mid   V=v_i, O =1, \mb k) \\
\pr(O_{V\leftarrow v_i} =1 \mid \bigvee_{v \not =  v_i}  \mb V=v, O=0 , \mb k) 
\label{eq:mpn}
\end{align}


\begin{definition}[Necessity and Sufficiency Scores]
  Given a probabilistic causal model $\pcm$, a decision-making algorithm $f: \mb X \rightarrow \{0,1\} $  a multivalued variable $V \in \mb V$ with $Dom(V) = \{v_1, v_2, \ldots, v_n\}$ and a set of
  variables $\mb K \subseteq \mb V-\{V,O\}$. We quantify the influence of an event $V=v_i$ to the decision made by
  $f$ for a sub-population  $\mb k \in Dom(\mb K)$ using the following scores:
  \begin{itemize}
  \item The {\em necessity score}:
    \begin{align} 
      N(v_i\mid \mb k) &=  \pr(\bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0 \mid V=v_i,  O=1, \mb K=\mb k) \label{eq:ns} 
    \end{align}
  \item The {\em sufficiency score}:
    \begin{align}
      S(v_i\mid \mb k) &= \sum_{v \not =  v_i}\pr(O_{V\leftarrow v_i}=1 \mid V=v, O=0, \mb K=\mb k) \label{eq:ps}
    \end{align}
  \item The {\em necessity and sufficiency score}:
    \begin{align} 
      NS(v_i\mid \mb k) &= \pr(O_{V\leftarrow v}=1, \bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0 \mid \mb K=\mb k) \label{eq:pns}
    \end{align}
  \end{itemize}
\end{definition}
%

\begin{prop} The necessity score, sufficiency score and necessity and sufficiency score are related thorough the following expression:
\begin{align}
    NS(V\mid \mb k)=\Pr(O=1, V=v \mid \mb k) N(V \mid k)+ \Pr(O=0, V=v' \mid \mb k) S(V \mid k)
\end{align}
\end{prop}

\begin{proof} The relationship obtained by applying the rule of total probability and consistency rules in the following steps:
{\small
  \begin{align}
    NS(v_i | \mb k)
    &= \frac{\pr(O_{V\leftarrow v_i}=1, \bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0, \mb k)}{\pr(\mb k)} \\
    &= \frac{1}{\pr(\mb k)} \sum_{x \in Dom(V)}
      \pr(O_{V\leftarrow v_i}=1, \bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0, \mb k, V=x) \\
    & = \frac{1}{\pr(\mb k)} \big(\pr(O_{V\leftarrow v_i}=1, \bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0 , \mb k, V=v_i)+
   \sum_{x \in Dom(V)-\{v\}}   \pr(O_{V\leftarrow v_i}=1, \bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0 , \mb k, V=x) \big)\\
    & = \frac{1}{\pr(\mb k)} \big(\pr(O=1, \bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0 , \mb k, V=v_i)+
   \sum_{x \in Dom(V)-\{v\}}   \pr(O_{V\leftarrow v_i}=1, \bigwedge_{v \not =  v_i \land x}  \ O_{V\leftarrow v} =0 , O=1, \mb k, V=x) \big)\\
       & \leq \frac{1}{\pr(\mb k)} \big(\pr(O=1, \bigwedge_{v \not =  v_i}  \ O_{V\leftarrow v} =0 , \mb k, V=v_i)+
   \sum_{x \in Dom(V)-\{v\}}   \pr(O_{V\leftarrow v_i}=1 , O=1, \mb k, V=x) \big)\\
    & \leq \Pr(O=1, V=v_i \mid \mb k) \ N(v_i \mid k)+ \Pr(O=0, V=v' \mid \mb k) \ S(V \mid k)
  \end{align}
 } 
\end{proof}



In the following, we introduce three commonly used probabilistic counterfactual
statements that follow from the notions of necessity and sufficiency in causal
reasoning.


\paragraph{Necessary and Sufficient Causation}

We assume that $X = \{x,x'\}$ is a binary protected attribute, where $x$
represents the privileged and $x'$ the non-privileged group. In addition,
$Y = \{y,y'\}$ is a binary outcome variable, where $y$ represents the ``good''
and $y'$ the ``bad'' outcome.

In the counterfactual account of necessary and sufficiency causation are defined
as follows:
\begin{itemize}
\item An event $X=x$ is a {\em necessary cause} of the event $Y=y$, if $Y=y$ had
not occurred in the absence of $X=y$, which translates to the following logical
statement: %
  \begin{align} \forall \mb u \ \ X(\mb u)=x \land Y(\mb u)=y \implies
Y_{x'}(\mb u)=y' \label{eq:ln}
  \end{align}
\item An event $X=x$ is a {\em sufficient cause} of the event $Y=y$ if in
situations where $X=x'$ and $X=x'$, had $X=x$ occurred, $Y$ would have been $y$,
which translates to the following logical statement:
  % 
  \begin{align} \forall \mb u \ \ X(\mb u)=x' \land Y(\mb u)=y' \implies
Y_{x}(\mb u)=y \label{eq:ls}
  \end{align}
  % 
\end{itemize}


\paragraph{Probability of Necessity and Sufficiency} We next present the
probabilistic variants of the logical implications for necessary and sufficient
causation~\cite{pearl2009causality}.

\begin{itemize}
\item \emph{Probability of Necessity:} The probability of necessity is the probabilistic
  interpretation of~\eqref{eq:ln}:
  \begin{align}
    PN = \pr(Y_{X \leftarrow x'} = y'| X=x, Y=y)  \label{eq:pn:orig}
  \end{align}

  In words, $PN$ computes how likely it is that $Y$ is equal to $y'$ (i.e., the
  bad outcome) if $X$ had been $x'$ (non-privileged group), given that $X=x$
  (privileged) and $Y=y$ (good outcome) did actually occur. In particular, if
  the implication \eqref{eq:ln} holds then $PN = 1$.

\item \emph{Probability of Sufficiency:} The probability of sufficiency is the probabilistic
  interpretation of~\eqref{eq:ls}:
  \begin{align}
    PS &= \pr(Y_{\mb x}=y| x',y') \label{eq:ps:orig}  
  \end{align}

  PS measures the capacity of $x$ to produce $y$, which implies that previously
  $x$ and $y$ were absent. If the implication \eqref{eq:ls} holds, then $PS = 1$.

  The probability of sufficiency has many applications in explanations, e.g., we
  can use PS to find the action $X = x$ that is most likely to produce the
  ``good'' outcome $Y = y$.

\item \emph{Probability of Necessity and Sufficiency:} The probability of
  necessity and sufficiency is defined as:
  \begin{align}
    PNS &= \pr(Y_{x}=y, Y_{x'}=y') \label{eq:pns:orig}  
  \end{align}

  PNS measures the probability that $Y$ responds to $X$ both ways, and thus
  measure both the sufficiency and necessity of $x$ to produce $y$.
\end{itemize}

% According to the counterfactual definition of necessary causation, the event
% $X=x$ is a necessary cause of the event $Y=y$, if $Y=y$ has not occurred in the
% absence of $X=y$, which translates to the following logical statement:
% \begin{align}
% \forall \mb u \ \  X(\mb u)=x \land  Y(\mb u)=y  \implies Y_{x'}(\mb u)=y' \label{eq:ln}
% \end{align}
% %
% The logical implication \eqref{eq:ln} has the following probabilistic
% implication:
% %
% \begin{align}
%   (\ref{eq:ln}) \  \Longleftrightarrow \ \pr(Y_{\mb x'}=y'| x,y)=1
% \end{align}
% %
% The quantify $\pr(Y_{\mb x'}=y'| x,y)$ is called {\em probability of necessity}, henceforth. 

% \paragraph{Probability of Necessity and Sufficiency} In the counterfactual account of necessary and sufficiency causation are defined as follows: 
% \begin{itemize}
% \item An event $X=x$ is a {\em necessary cause} of the event $Y=y$, if $Y=y$ had not occurred in the absence of $X=y$, which translates to the following logical statement: %
% \begin{align}
% \forall \mb u \ \  X(\mb u)=x \land  Y(\mb u)=y  \implies Y_{x'}(\mb u)=y' \label{eq:ln}
% \end{align}
% \item An event $X=x$ is a {\em sufficient cause} of the event $Y=y$ if in situations where $X=x'$ and $X=x'$, had $X=x$ occurred, $Y$ would have been $y$, which translates to the following logical statement: 
% %
% \begin{align}
% \forall \mb u \ \  X(\mb u)=x' \land  Y(\mb u)=y'  \implies Y_{x}(\mb u)=y \label{eq:ls}
% \end{align}
% %
% \end{itemize}

% The logical implications (\ref{eq:ln}) and (\ref{eq:ls}) have the following probabilistic implications:
% %
% \begin{align}
% (\ref{eq:ln}) \  &\Longleftrightarrow \ \pr(Y_{\mb x'}=y'\mid x,y)=1 \\
% (\ref{eq:ls}) \  &\Longleftrightarrow \ \pr(Y_{\mb x}=y \mid x',y')=1
% \end{align}
% %
% The quantifies $\pr(Y_{\mb x'}=y'| x,y)$ and $\pr(Y_{\mb x}=y| x',y')$ are respectively called {\em probability of necessity} and {\em probability of sufficiency}, henceforth.


\ignore{
  % \paragraph{Probability of Necessity}
  % According to the counterfactual definition of necessary causation, the event
  % $X=x$ is a necessary cause of the event $Y=y$, if $Y=y$ does not occur in the
  % absence of $X=x$, which translates to the following logical statement:
  % % 
  % \begin{align}
  %   \forall \mb u \ \ X(\mb u)=x \land  Y(\mb u)=y  \implies Y_{x'}(\mb u)=y' \label{eq:pn:logical}
  % \end{align}
  % % 
  % Probability of necessity is just the sum of the probability of all $\mb u$ in
  % which (\ref{eq:pn:logical}) holds or equivalently:

  % \begin{align}
  %   PN
  %   &=1- \sum_{\{\mb u \mid X(\mb u)=x \land Y(\mb u)=y \land Y_{\mb x'}(\mb u)=y \}} \pr(\mb u) \\
  %   &= 1- \sum_{\mb u} \ \pr(Y_{\mb x'}(\mb u)=y) \pr(\mb u|x,y) \\
  %   &=1- \pr(Y_{\mb x'}=y| x,y) \\
  %   &=\pr(Y_{x'}=y'| x,y) \label{eq:pn:orig} \\
  %   &=\sum_{\mb u} \ \pr(Y_{x'}(\mb u)=y') \pr(\mb u | x,y) 
  % \end{align}
}


Bounding and estimating the explanation scores using results established in this paper rely on the existence of background knowledge. However, our system \sys\ is designed to work with any level of user's background knowledge. If no background knowledge is provided, \sys\ assumes $\pr(o \mid \Do(\mb \mb x), \mb k)=\pr(o \mid \mb \mb x, \mb k)$ and monotonicity.  Under these assumptions: the necessity score becomes $\frac{  \pr(o' \mid \mb z',\mb k)  - \pr(o' \mid \mb z,\mb k) }{\pr(o \mid \mb z,   \mb k)}$ that can be seen as group-level {\em attributable fraction} which is  widely used in epidemiology as a measure of the proportion of cases attributed to a particular risk factor~\cite{poole2015history}; The sufficiency score becomes $\frac{\pr(o\mid  \mb z ,\mb k) - \pr(o\mid \mb z', \mb k) }{\pr(o' \mid  \mb z', \mb k)}$ that can be seen as group-level {\em relative risk} which is widely used in epidemiology to measure the risk of contracting a disease in a group exposed to a risk factor~\cite{khoury1989measurement};  and the necessity and sufficiency score becomes 
$\pr(o \mid \mb z, \mb k)-\pr(o \mid \mb z',  \mb k)$ which, when measured for sensitive attributes such as race or gender, is known as {\em conditional statistical parity} in the fairness literature~\cite{corbett2017algorithmic}. 

==> exp.tex <==
\section{Counterfactual Explanations and Recourse}

In this section, based on the scores defined in Section~\ref{sec:scores} we generate two types of explanations for ML algorithms. 
















==> extensions.tex <==
\revision{\section{Further Extensions}
\romila{We can probably combine both extensions into one.}
Mention:Ordering is not restrictive!
\noindent \textbf{Extension to multi-class classification.} Consider the case when the outcome is multi-valued, i.e.,  $Dom(O) = \{o_1, \ldots, o_{\gamma}\}$ where $o_1 >  \ldots > o_{\gamma}$ represents an ordering of the values such that $o_i > o_j$ implies that $o_i$ is more desirable than $o_j$. We redefine the explanation scores in terms of each outcome value as follows: 
\begin{itemize}
  \item Necessity score is defined as the probability that the outcome $O$ changes from a value $o_j\geq o$ to a lower value $o' < o$ upon the intervention $X \leftarrow x'$: 
  \begin{align*} 
       \nec_{x}^{x'}(\mb k, o) &\defeq \pr(\underset{o'<o}{\cup} o'_{X \leftarrow x'} \mid x,  \underset{o^j\geq o}{\cup} o^j, \mb k) 
    %   = \sum_{o' < o} \pr(o'_{X \leftarrow x'} \mid x, o, \mb k)
    \end{align*}
  \item Sufficiency score is defined as the probability that $O$ changes from a value $o' \leq o$ to a higher value $o_j > o$ upon the intervention $X \leftarrow x'$:
  {   \begin{align*} 
      \suf_x^{x'}(\mb k, o) & \defeq \pr(\underset{o^j \geq o}{\cup} o'_{X\leftarrow x} \mid x', \underset{o' < o}{\cup}o', \mb k) 
    \end{align*}}
  \item Necessity and sufficiency score is defined as the probability that the intervention $X \leftarrow x$ results in a higher value $o^j \geq o$ whereas $X \leftarrow x'$ results in a lower value $o' < o$:
     {  \begin{align*}  
    \nsuf_x^{x'}(\mb k) &\defeq \pr(\underset{o^j \geq o}{\cup} o^j_{X\leftarrow x}, \underset{o'<o}{\cup} o'_{X\leftarrow x'} \mid \mb k)
    \end{align*}}
  \end{itemize}
  The scores, thus defined, can be estimated using Proposition~\ref{prop:iden:mon:ci}.
  
\noindent \textbf{Extension to regression.} We can similarly define the scores for continuous-valued outcomes at each outcome value. In other words, for an outcome $o$, we partition the domain of outcome values as $o^j \geq o$ and $o' < o$. The explanation scores are then defined as:
\begin{itemize}
  \item Necessity score is defined as the probability that the outcome $O$ changes from a value $o_j\geq o$ to a lower value $o' < o$ upon the intervention $X \leftarrow x'$: 
  \begin{align*} 
       \nec_{x}^{x'}(\mb k, o) &\defeq \pr(o'_{X \leftarrow x'} \mid x,  o^j, \mb k) 
    %   = \sum_{o' < o} \pr(o'_{X \leftarrow x'} \mid x, o, \mb k)
    \end{align*}
  \item Sufficiency score is defined as the probability that $O$ changes from a value $o' \leq o$ to a higher value $o_j > o$ upon the intervention $X \leftarrow x'$:
  {   \begin{align*} 
      \suf_x^{x'}(\mb k, o) & \defeq \pr(o'_{X\leftarrow x} \mid x', o', \mb k) 
    \end{align*}}
  \item Necessity and sufficiency score is defined as the probability that the intervention $X \leftarrow x$ results in a higher value $o^j \geq o$ whereas $X \leftarrow x'$ results in a lower value $o' < o$:
     {  \begin{align*}  
    \nsuf_x^{x'}(\mb k) &\defeq \pr(o^j_{X\leftarrow x}, o'_{X\leftarrow x'} \mid \mb k)
    \end{align*}}
  \end{itemize}

}

==> missingproof.tex <==












\begin{proof} %The proof is similar to the proof of Proposition~\ref{prop:iden:mon:bounds} and obtained by incorporating Equation~\eqref{eq:backdoor} and  the fact that under monotonicity $\pr(o'_{\mb X\leftarrow \mb x}, o_{\mb X\leftarrow \mb x'}, \mb x,\mb k)=0$.
{
Here, we only prove \eqref{eq:nec:mon:ident}. The proof of \eqref{eq:suff:mon:ident} and \eqref{eq:nec:nsuff:ident} are similar. Notice that monotonicity implies $\pr(o'_{\mb X\leftarrow \mb x}, o_{\mb X\leftarrow \mb x'}, \mb x,\mb k)=0$. Also note that if $\mb C \cup \mb K$ satisfies  the backdoor-criterion, then the following independence, known as conditional ignorability, holds: $(O_{\mb X\leftarrow \mb x} \indep \mb X \mid \mb C \cup \mb K)$\cite{pearl2016causal}[Theorem 4.3.1]. We show \eqref{eq:nec:mon:ident} in the following steps:}
%
{\scriptsize
  \begin{align}
    \nec_{\mb x}(\mb k)
    &= \frac{\pr(o'_{X \leftarrow \mb x'}, \mb x,  o, \mb k)}{\pr(o, \mb x, \mb k)}= \frac{\pr(o'_{\mb X\leftarrow \mb x'} \mid \mb x,\mb k) - \pr(o' \mid \mb x,\mb k) }{\pr(o \mid \mb x,   \mb k)} \\& \hspace{3.2cm}\texttt{(from Eq.~\eqref{proof:bound:4}, ~\eqref{eq:consistency} and monotonicity)}\nonumber  \\ 
    &= \frac{\sum_{c\in Dom(C)} \pr(o'_{\mb X\leftarrow \mb x'} \mid  \mb c, \mb x,\mb k) \ \pr(\mb c \mid \mb x, \mb k)  - \pr(o' \mid \mb x,\mb k) }{\pr(o \mid \mb x,   \mb k)}\nonumber \\        
    &= \frac{\sum_{c\in Dom(C)} \pr(o' \mid \mb c,\mb x',\mb k) \ \pr(\mb c \mid \mb x, \mb k)  - \pr(o' \mid \mb x,\mb k) }{\pr(o \mid \mb x,   \mb k)} \nonumber \\ & \hspace{2.4cm}  \texttt{(from conditional ignorability and Eq.~\eqref{eq:consistency})} \nonumber
  \end{align}
}
\end{proof}
